Multi-Vector Models with Textual Guidance for Fine-Grained Scientific Document Similarity

We present a new scientific document similarity model based on matching fine-grained aspects of texts. To train our model, we exploit a naturally-occurring source of supervision: sentences in the full-text of papers that cite multiple papers together (co-citations). Such co-citations not only reflect close paper relatedness, but also provide textual descriptions of how the co-cited papers are related. This novel form of textual supervision is used for learning to match aspects across papers. We develop multi-vector representations where vectors correspond to sentence-level aspects of documents, and present two methods for aspect matching: (1) A fast method that only matches single aspects, and (2) a method that makes sparse multiple matches with an Optimal Transport mechanism that computes an Earth Mover's Distance between aspects. Our approach improves performance on document similarity tasks in four datasets. Further, our fast single-match method achieves competitive results, paving the way for applying fine-grained similarity to large scientific corpora. Code, data, and models available at: https://github.com/allenai/aspire

==> floats/tables/ablation-scib-spec.tex <==
\begin{table}[h!]
\centering
\scalebox{0.7}{
\begin{tabular}{rcc}
 & \multicolumn{2}{c}{\shortstack[c]{\textsc{CSFCube}\\\textit{Aggregated}}}\\
 & MAP   & NDCG$_{\%20}$  \\\hline
\texttt{MultiInst$_\mathtt{SciB}$}        & $\underset{\pm 1.37}{36.66}$ & $\underset{\pm 0.86}{57.68}$\\
\texttt{MultiInst$_\mathtt{Spec}$}        & $\underset{\pm 1.38}{\bf 39.42}$ & $\underset{\pm 1.53}{\bf 60.63}$\\
\end{tabular}}\\
\scalebox{0.7}{
\begin{tabular}{rcccc}
 & \multicolumn{2}{c}{\textsc{treccovid}$_\mathtt{RF}$} 
 & \multicolumn{2}{c}{\textsc{relish}}\\
 &  MAP  & NDCG$_{\%20}$ & MAP  & NDCG$_{\%20}$  \\\hline
\texttt{MultiInst$_\mathtt{SciB}$}        & $\underset{\pm 1.15}{24.87}$ & $\underset{\pm 1.49}{54.33}$ & $\underset{\pm 0.31}{61.36}$ & $\underset{\pm 0.24}{78.10}$\\
\texttt{MultiInst$_\mathtt{Spec}$}        & $\underset{\pm 0.85}{\bf 25.84}$ & $\underset{\pm 1.21}{\bf 56.52}$ & $\underset{\pm 0.97}{61.20}$ & $\underset{\pm 0.36}{78.00}$\\
%\texttt{Expl$_\mathtt{SciB}$}             & $\underset{\pm 0.76}{40.10}$ & $\underset{\pm 0.61}{60.92}$ & $\underset{\pm 0.71}{27.68}$ & $\underset{\pm 0.75}{58.42}$ & $\underset{\pm 0.31}{61.45}$ & $\underset{\pm 0.33}{78.12}$\\
%\texttt{Expl$_\mathtt{Spec}$}             & $\underset{\pm 0.93}{40.26}$ & $\underset{\pm 0.67}{60.71}$ & $\underset{\pm 0.45}{26.24}$ & $\underset{\pm 0.65}{56.55}$ & $\underset{\pm 0.51}{61.29}$ & $\underset{\pm 0.42}{77.89}$
\end{tabular}}
\caption{Performance of fine-grained similarity model trained with multi-instance learning, with SciBERT vs Specter initialization.}
\label{tab-scib-spec-finegrained}
\end{table}

==> floats/tables/ablation-tables.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{rcccccc}
 & \multicolumn{2}{c}{\shortstack[c]{\textsc{CSFCube}\\\textit{Aggregated}}}
 & \multicolumn{2}{c}{\textsc{treccovid}$_\mathtt{RF}$} 
 & \multicolumn{2}{c}{\textsc{relish}}\\
 & MAP   & NDCG$_{\%20}$    &  MAP  & NDCG$_{\%20}$ & MAP  & NDCG$_{\%20}$  \\\hline
\texttt{MultiInst$_\mathtt{SciB}$}        & $\underset{\pm 1.37}{36.66}$ & $\underset{\pm 0.86}{57.68}$ & $\underset{\pm 1.15}{24.87}$ & $\underset{\pm 1.49}{54.33}$ & $\underset{\pm 0.31}{61.36}$ & $\underset{\pm 0.24}{78.10}$\\
\texttt{MultiInst$_\mathtt{Spec}$}        & $\underset{\pm 1.38}{39.42}$ & $\underset{\pm 1.53}{60.63}$ & $\underset{\pm 0.85}{25.84}$ & $\underset{\pm 1.21}{56.52}$ & $\underset{\pm 0.97}{61.20}$ & $\underset{\pm 0.36}{78.00}$\\
\texttt{Expl$_\mathtt{SciB}$}             & $\underset{\pm 0.76}{40.10}$ & $\underset{\pm 0.61}{60.92}$ & $\underset{\pm 0.71}{27.68}$ & $\underset{\pm 0.75}{58.42}$ & $\underset{\pm 0.31}{61.45}$ & $\underset{\pm 0.33}{78.12}$\\
\texttt{Expl$_\mathtt{Spec}$}             & $\underset{\pm 0.93}{40.26}$ & $\underset{\pm 0.67}{60.71}$ & $\underset{\pm 0.45}{26.24}$ & $\underset{\pm 0.65}{56.55}$ & $\underset{\pm 0.51}{61.29}$ & $\underset{\pm 0.42}{77.89}$
\end{tabular}
\caption{Performance of fine-grained similarity models with SciBERT vs Specter initialization.}
\label{tab-scib-spec-finegrained}
\end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{rcccccc}
 & \multicolumn{2}{c}{\shortstack[c]{\textsc{CSFCube}\\\textit{Aggregated}}}
 & \multicolumn{2}{c}{\textsc{treccovid}$_\mathtt{RF}$} 
 & \multicolumn{2}{c}{\textsc{relish}}\\
 & MAP   & NDCG$_{\%20}$    &  MAP  & NDCG$_{\%20}$ & MAP  & NDCG$_{\%20}$  \\\hline
\texttt{Expl$_\mathtt{Spec}$}             & $\underset{\pm 0.93}{40.26}$ & $\underset{\pm 0.67}{60.71}$ & $\underset{\pm 0.45}{26.24}$ & $\underset{\pm 0.65}{56.55}$ & $\underset{\pm 0.51}{61.29}$ & $\underset{\pm 0.42}{77.89}$\\
\texttt{AbsAli-Expl$_\mathtt{Spec}$}             & $\underset{\pm 1.39}{37.03}$ & $\underset{\pm 0.76}{59.57}$ & $\underset{\pm 0.9}{25.42}$ & $\underset{\pm 0.55}{55.34}$ & $\underset{\pm 0.69}{58.78}$ & $\underset{\pm 0.57}{75.80}$\\
\end{tabular}
\caption{Performance of fine-grained similarity model trained with weak supervision from explanations ablated for the effect of explanations vs influence of encoder model ($\mathtt{BERT}_{\mathcal{E}}$=\texttt{CoSentBert}; detailed in \S\ref{sec-fine-grained-data} and \ref{sec-model}) used to compute alignments to the explanation.}
\label{tab-finegrained-absali}
\end{table*}

\begin{table*}[t]
\centering
\begin{tabular}{rcccccc}
 & \multicolumn{2}{c}{\shortstack[c]{\textsc{CSFCube}\\\textit{Aggregated}}}
 & \multicolumn{2}{c}{\textsc{treccovid}$_\mathtt{RF}$} 
 & \multicolumn{2}{c}{\textsc{relish}}\\
 & MAP   & NDCG$_{\%20}$    &  MAP  & NDCG$_{\%20}$ & MAP  & NDCG$_{\%20}$  \\\hline
\texttt{OTAlign$_\mathtt{Spec}$}             & $\underset{\pm 0.53}{ 40.79}$ & $\underset{\pm 0.52}{61.41}$ & $\underset{\pm 0.53}{30.92}$ & $\underset{\pm 0.67}{62.23}$ & $\underset{\pm 0.29}{62.57}$ & $\underset{\pm 0.26}{78.95}$\\
\texttt{AttAlign$_\mathtt{Spec}$}      & $\underset{\pm 1.52}{41.85}$ & $\underset{\pm 0.82}{61.67}$ & $\underset{\pm 0.78}{29.51}$ & $\underset{\pm 0.51}{60.96}$ & $\underset{\pm 0.52}{61.92}$ & $\underset{\pm 0.50}{78.54}$\\
\end{tabular}
\caption{Attention aggregation instead of optimal transport alignment.}
\label{tab-attention-align}
\end{table*}

\begin{table}[t]
\centering
%\rowcolors{15}{gray!25}{white}
\scalebox{0.67}{
\begin{tabular}{rcc|cc}
& \multicolumn{2}{c}{\textsc{treccovid}$_\mathtt{RF}$}   & \multicolumn{2}{c}{\textsc{relish}}        \\
& MAP   & NDCG$_{\%20}$    &  MAP  & NDCG$_{\%20}$  \\\hline
\texttt{SentBert-1B}  & 17.35 & 43.87 & 52.92 & 69.69\\\hline
\texttt{SentBert-PP}  & 11.12 & 34.85 & 50.80 & 67.35\\
\texttt{SentBert-NLI} & 13.43 & 40.78 & 47.02 & 63.56\\
\texttt{UnSimCSE-BERT}  & 9.85  & 34.27 & 45.79 & 62.02\\
\texttt{SuSimCSE-BERT}  & 11.50 & 37.17 & 47.29 & 63.93\\
\texttt{CoSentBert}     & 12.80 & 38.07 & 50.04 & 66.35\\
\texttt{ICTSentBert}    & 9.80  & 33.62 & 47.72 & 63.71\\\hline
\texttt{Specter}        & 28.24 & 59.28 & 60.62 & 77.20\\
\texttt{Specter-CoCite$_\mathtt{Scib}$}    & $\underset{\pm 0.87}{30.60}$ & $\underset{\pm 0.95}{62.07}$ & $\underset{\pm 0.32}{61.43}$ & $\underset{\pm 0.1}{78.01}$\\
\texttt{Specter-CoCite$_\mathtt{Spec}$}    & $\underset{\pm 0.25}{28.59}$ & $\underset{\pm 0.36}{60.07}$ & $\underset{\pm 0.24}{61.43}$ & $\underset{\pm 0.23}{77.96}$\\\hline
\texttt{MultiInst$_\mathtt{Scib}$}         & $\underset{\pm 1.15}{24.87}$ & $\underset{\pm 1.49}{54.33}$ & $\underset{\pm 0.31}{61.36}$ & $\underset{\pm 0.24}{78.10}$\\
\texttt{Expl$_\mathtt{Scib}$}            & $\underset{\pm 0.71}{27.68}$ & $\underset{\pm 0.75}{58.42}$ & $\underset{\pm 0.31}{61.45}$ & $\underset{\pm 0.33}{78.12}$\\
\texttt{Expl+MultiInst$_\mathtt{Scib}$}  & $\underset{\pm 1.01}{28.68}$ & $\underset{\pm 0.87}{58.88}$ & $\underset{\pm 0.16}{62.32}$ & $\underset{\pm 0.02}{78.78}$\\
\texttt{OTAlign$_\mathtt{Scib}$}         & $\underset{\pm 0.68}{30.03}$ & $\underset{\pm 0.75}{61.74}$ & $\underset{\pm 0.34}{62.24}$ & $\underset{\pm 0.31}{78.78}$\\
\texttt{Expl+OTAlign$_\mathtt{Scib}$}    & $\underset{\pm 1.17}{31.95}$ & $\underset{\pm 1.35}{63.14}$ & $\underset{\pm 0.39}{62.32}$ & $\underset{\pm 0.23}{78.77}$\\
\end{tabular}
}
\caption{Test set results for baseline and proposed methods. Metrics
(MAP, NDCG$_{\%20}$) are computed based averages over three re-runs of models. 
Standard deviations are below run averages.}
\label{tab-model-results-biomed-scib}
\end{table}

==> floats/tables/baselines-miexplot-scid.tex <==
\begin{table*}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
SciDocs tasks $\rightarrow$ & 
\multicolumn{2}{c}{\texttt{Citations}}   &
\multicolumn{2}{c}{\texttt{Co-Citations}}       & 
\multicolumn{2}{c}{\texttt{Co-Reads}}       &
\multicolumn{2}{c}{\texttt{Co-Views}}           \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
Models & MAP   & NDCG     &  MAP  & NDCG & MAP   & NDCG     &  MAP  & NDCG  \\\midrule
 \textsc{MPNet-1B}            & 86.76 & 92.63 & 85.68 & 92.16 & 83.45 & 90.47 & 82.51 & 89.29\\\midrule
 \textsc{Specter}                & \textbf{92.39} & \textbf{95.90} & 88.32 & 93.88 & 86.42 & 92.39 & 84.65 & 90.70\\
 \textsc{Specter-CoCite$_\mathtt{Scib}$}   & ${89.16}$ & ${93.97}$ & ${90.21}$ & ${94.76}$ & ${86.85}$ & ${92.51}$ & ${85.70}$ & ${91.37}$\\
 \textsc{Specter-CoCite$_\mathtt{Spec}$}   & ${89.85}$ & ${94.26}$ & ${90.82}$ & ${95.11}$ & ${87.14}$ & ${92.65}$ & ${85.81}$ & ${91.35}$\\\midrule
%  \textsc{MultiInst$_\mathtt{Spec}$}        & ${90.89}$ & ${94.95}$ & ${90.69}$ & ${95.15}$ & ${87.39}$ & ${92.86}$ & ${85.74}$ & ${91.37}$\\
\textsc{ts\aspect}$_\mathtt{Spec}$             & ${90.99}$ & ${95.04}$ & ${\bf 90.92}$ & ${\bf 95.26}$ & ${87.51}$ & ${92.97}$ & ${\bf 85.87}$ & ${\bf 91.46}$\\
%  \textsc{Expl+MultiInst$_\mathtt{Spec}$}   & ${91.11}$ & ${94.99}$ & ${90.91}$ & ${95.25}$ & ${\bf 87.65}$ & ${\bf 92.99}$ & ${\bf 85.95}$ & ${\bf 91.46}$\\
\textsc{ot\aspect}$_\mathtt{Spec}$          & ${91.13}$ & ${95.08}$ & ${90.88}$ & ${95.25}$ & ${87.50}$ & ${92.90}$ & ${85.70}$ & ${91.30}$\\
\textsc{ts+ot\aspect}$_\mathtt{Spec}$     & ${91.09}$ & ${95.03}$ & ${90.83}$ & ${95.22}$ & ${\bf 87.60}$ & ${\bf 92.98}$ & ${85.81}$ & ${91.42}$\\\bottomrule
\end{tabular}
}
\caption{Test set results for baseline and proposed methods on sub-tasks included in the \textsc{SciDocs} benchmark. Our approaches outperform a prior strong model,  \textsc{Specter}, by 1-1.5 points on 3 of 4 sub-tasks. Metrics (MAP, NDCG) are computed based on averages over three re-runs of models.  \textsc{Specter} uses model parameters as part of the Huggingface library. Here, \textsc{ts\aspect}: Text supervised single-match method, \textsc{ot\aspect}: Optimal Transport multi-match method and \textsc{ts+ot\aspect}: Multi-task multi aspect method.}
\label{tab-model-results-scidocs}
\end{table*}
